Width, depth and space

The width measure treedepth, also known as vertex ranking, centered coloring and elimination tree height, is a well-established notion which has recently seen a resurgence of interest. Since graphs of bounded treedepth are more restricted than graphs of bounded tree- or pathwidth, we are interested in the algorithmic utility of this additional structure. On the negative side, we show that every dynamic programming algorithm on treedepth decompositions of depth~$t$ cannot solve Dominating Set with $O((3-\epsilon)^t \cdot \log n)$ space for any $\epsilon > 0$. This result implies the same space lower bound for dynamic programming algorithms on tree and path decompositions. We supplement this result by showing a space lower bound of $O((3-\epsilon)^t \cdot \log n)$ for 3-Coloring and $O((2-\epsilon)^t \cdot \log n)$ for Vertex Cover. This formalizes the common intuition that dynamic programming algorithms on graph decompositions necessarily consume a lot of space and complements known results of the time-complexity of problems restricted to low-treewidth classes. We then show that treedepth lends itself to the design of branching algorithms. This class of algorithms has in general distinct advantages over dynamic programming algorithms: a) They use less space than algorithms based on dynamic programming, b) they are easy to parallelize and c) they provide possible solutions before terminating. Specifically, we design for Dominating Set a pure branching algorithm that runs in time $t^{O(t^2)}\cdot n$ and uses space $O(t^3 \log t + t \log n)$ and a hybrid of branching and dynamic programming that achieves a running time of $O(3^t \log t \cdot n)$ while using $O(2^t t \log t + t \log n)$ space. Algorithms for 3-Coloring and Vertex Cover with space complexity $O(t \cdot \log n)$ and time complexity $O(3^t \cdot n)$ and $O(2^t\cdot n)$, respectively, are included for completeness.

==> header.tex <==
% FONTS and SYMBOLS
\usepackage{bbm}
\usepackage{mathrsfs}
\usepackage{latexsym}
\usepackage{paralist}
\usepackage{mathdots}

% LATEX stuff
\usepackage{suffix}

% TYPOGRAPHY
\usepackage{xpunctuate}
\usepackage[all]{foreign} % Typesets abbreviations like e.g.
\usepackage{xfrac} % Nice in-text fractions

% MATHEMATICS
\usepackage{amsfonts,amssymb,amstext,amsthm} % AMS packages
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{thm-restate}

\usepackage[full,small]{complexity}

% FIGURES
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}


% DEBUGGING
\providecommand*\showkeyslabelformat[1]{%
\rotatebox{279}{{\normalfont{\textsf{#1}}}}}
\usepackage[notref,color,final]{showkeys} % Use option 'final' to remove

% TOOLS
\usepackage{xargs}

% COLORS and GRAPHICS
\PassOptionsToPackage{dvipsnames,usenames,table}{xcolor}
\usepackage{tikz}
% \usetikzlibrary{arrows,shapes}
% \usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{calc}

% FIGURES and TABLES and LISTS
\usepackage{booktabs} % Better tables
\usepackage{longtable}
\usepackage{float}
\usepackage{wrapfig}
\usepackage{floatflt}
\usepackage{framed}
\usepackage{ctable}

\def\figscale{.7}
\def\smallfigscale{.5}

\usepackage{enumerate}
\usepackage{enumitem}
\usepackage{xspace}
\usepackage{xifthen}
\usepackage{fixltx2e}
\usepackage{url}
\usepackage{scrtime}
\usepackage{tikz}

% Debugging
%\setlength\overfullrule{5pt} % For debugging overfull lines


% Nice little hack to output time spend per page (grep for 'timer' in log)
\usepackage{atbegshi}
\newcommand\showtimer{%
  \message{^^Jtimer: \the\numexpr\the\pdfelapsedtime*1000/65536\relax}%
  \pdfresettimer}
\AtBeginDocument{\showtimer}
\AtBeginShipout {\showtimer}

% Algorithms
% \usepackage[longend,vlined]{algorithm2e}
% \renewcommand\AlCapFnt{\normalfont\small} % Make consistent w/ classicthesis
% \renewcommand\AlCapNameSty{\normalfont\small} 
\usepackage{algorithm} 
\usepackage{algpseudocode}                     
%\usepackage{subfigure}
\input{epsf}

% MARGIN NOTES
\usepackage{xkvltxp}
\usepackage[footnote,draft,english,silent,nomargin]{fixme}
\newcommand{\todo}[1]{\fxfatal{\color{red}#1}}
\newcommand{\warn}[1]{\fxwarning{#1}}
\newcommand{\note}[1]{\fxnote{#1}}

% Indexing
\usepackage{index}

\makeindex
\newindex{sym}{sym.idx}{sym.ind}{Symbol index}
\newindex{prob}{prob.idx}{prob.ind}{Problem index}

\newcommand\iemph[1]{\emph{#1}\index{#1|textbf}}
\newcommand\mathindex[1]{\index[sym]{\ensuremath{{#1}}}}
\WithSuffix\newcommand\mathindex*[1]{\index*[sym]{{#1}}}

% Nice little command to modify sub- and superscripts.
% Usage: \raisemath{2pt}{...}
% see http://tex.stackexchange.com/questions/5191/how-to-raise-a-subscript
\makeatletter
\newcommand{\raisemath}[1]{\mathpalette{\raisem@th{#1}}}
\newcommand{\raisem@th}[3]{\raisebox{#1}{$#2#3$}}
\makeatother

% Typesetting of important things
\def\N{\mathbb{N}} % Natural numbers
% \def\R{\mathbb{R}}	% Real numbers % Not needed so far.
\def\Rp{\mathbb{R^+}}
\def\Z{\mathbb{Z}}	% Integers
\def\Q{\mathbb{Q}}	% Fractions

\renewcommand{\cal}{\mathcal}

\newcommand{\name}[1]{\textsc{#1}}
\newcommand{\rem}[1]{\textcolor{red}{[#1]}}
\newcommand{\modif}[1]{\textcolor{blue}{#1}}
\newcommand{\xtof}[1]{\textcolor{blue}{[Xtof: #1]}}

\newcommand{\mc}{\mathcal}
\newcommand{\mb}{\mathbf}
\newcommand{\mbb}{\mathbb}

\newcommand{\ind}{\subseteq_{ind}}
\newcommand{\indprop}{\subsetneq_{ind}}

\newcommand{\planarF}{\textsc{Planar-$\mc{F}$-Deletion}}
\newcommand{\DplanarF}{\textsc{Disjoint Planar-$\mc{F}$-Deletion}}

\newcommand\Problem[2][]{%
  \ifthenelse{\isempty{#1}}{%
    \textsc{#2}\index[prob]{#2@\textsc{#2}}\xspace
  }{%
    \textsc{#1}\index[prob]{#2@\textsc{#2}}\xspace
  }
}
\WithSuffix\newcommand\Problem*[1]{\textsc{#1}\xspace} % Surpress indexing
\newcommand{\VC}{\Problem{Vertex Cover}}
\newcommand{\DS}{\Problem{Dominating Set}}
\newcommand{\ConnDS}{\Problem{Connected Dominating Set}}
\newcommand{\FVS}{\Problem{Feedback Vertex Set}}
\newcommand{\CVD}{\Problem{Chordal Vertex Deletion}}

\newcommand\overbar[2][3]{{}\mkern#1mu\overline{\mkern-#1mu#2}}
\def\comp#1{\overbar #1} % Complement
\newcommand\restr[2]{{% Restriction of functions, set families
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}

% Common math and typography
\def\half{{\sfrac{1}{2}}} % Needs second block to work as subscript
\def\third{{\sfrac{1}{3}}} % Needs second block to work as subscript
\def\twothird{{\sfrac{2}{3}}} % Needs second block to work as subscript
\def\threehalf{{\sfrac{3}{2}}} % Needs second block to work as subscript


% Graph operations & relations
\def\isom{\simeq}
\def\subgraph{\subseteq}
\def\isubgraph{\subseteq_i}
\def\minor{\preccurlyeq_{{\mathsf{m}}}\!} % Minor relation
\def\immersion{\preccurlyeq_{\mathsf{i}}\!} % Immersion relation
\def\tminor{\preccurlyeq_{\mathsf{t}}\!} % Top. minor relation
\def\sminor^#1{
    \preccurlyeq_{\mathrlap{\mathsf{m}}}^{#1}
} % Shallow minor relation
\def\ssminor^#1{%
    \mathbin{\dot\preccurlyeq_{{\mathrlap{\mathsf{m}}}}^{#1}}\,
} % Stable shallow minor relation
\def\stminor^#1{
    \preccurlyeq_{\mathrlap{\mathsf{t}}}^{#1}
} % Shallow minor relation
\def\sstminor^#1{%
    \mathbin{\dot\preccurlyeq_{{\mathrlap{\mathsf{t}}}}^{#1}}\,
} % Stable shallow top. minor relation


\def\forb{\operatorname{Forb}}

\def\adj{\operatorname{adj}}
\def\inc{\operatorname{inc}}
\def\arc{\operatorname{arc}}

% Colorings
\def\col{\mathsf{c}}

%\def\mathcolor#1{\ensuremath{\mathsf{#1}}\xspace}
%\def\black{\mathcolor{b}}
%\def\red{\mathcolor{r}}

% Graph operators
\newcommand*{\Cdot}{\raisebox{-.9ex}{\scalebox{2.75}{$\cdot$}}}
\def\lexprod{\mathbin{ \Cdot }}
\def\cjoin{ \mathbin{ \,\ast\, } }
\def\nullgraph{\varnothing}


% \usepackage{scalerel}
% \def\customnabla{\scalerel*{\includegraphics{fonts/grad}}{\nabla}}
% \def\wavynabla{\scalerel*{\includegraphics{fonts/topgrad}}{\nabla}}

\def\dir#1{\vec{#1}}
\def\grad_#1{\nabla\!_{#1}}
\def\sgrad_#1{{\dot\nabla}\!_{#1}}
\def\topgrad_#1{\widetilde \nabla\!_{#1}}
\def\stopgrad_#1{\dot{\widetilde\nabla}\!_{#1}}
\def\topomega_#1{\widetilde \omega_{#1}}

\def\colnum_#1{ \operatorname{col}_{#1} }
\def\wcolnum_#1{ \operatorname{wcol}_{#1} }

\def\symdiff{\mathop{\bigtriangleup}}
\DeclareMathOperator{\cliquegrad}{\square}

% \newcommand{\cliques}{\mathop{cliques}}  % Set of all cliques
\DeclareMathOperator{\centers}{centers}  % Set of all centers

\newcommand{\bnd}{\ensuremath{{\partial}}}    % Boundary symbol for t-boundaried graphs

% \newcommand{\tbnd}{\widetilde}   % Accent for t-boundaried graphs
%\newcommand{\tbnd}{\prescript{\color{black!33}\circ\!}{}}   % Accent for t-boundaried graphs
\newcommand{\tbnd}{%
  \mathchoice%
  {\raisebox{4.5pt}{{\scriptsize$\circ$}}\mkern-2mu} % displaystyle
  {\raisebox{4.5pt}{{\scriptsize$\circ$}}\mkern-2mu} % textstyle
  {\raisebox{4.1pt}{{\tiny$\circ$}}\mkern-3mu} % scriptstyle
  {\raisebox{4.5pt}{{\scriptsize$\circ$}}\mkern-2mu} % scriptscriptstyle
}

\newcommand{\Gt}{\tbnd G} 
\newcommand{\Ht}{\tbnd H}

\newcommand{\equipi}[1]{\ensuremath{\equiv_{\Pi,#1}}} 
        % Equivalence for t-boundaried graphs with t as parameter
\newcommand{\repsize}{\ensuremath{\rho}}   % Prot. repr. size
% \newcommand{\protd}{\ensuremath{\rho'}} % Prot. repr. size with doubled parameter

% Replace leq, geq by nicer variants
\renewcommand{\le}{\leqslant}
\renewcommand{\leq}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\geq}{\geqslant}

% A 0-dimension prime
\newcommand{\silentprime}{\,\mathclap{{}^{\smash \prime}}}

% Probabilities
\def\P{\mathbb P}
\def\E{\mathbb E}
\def\Var{\operatorname{Var}}


% Boundaried graphs, WQO, FII, replacement
\DeclareMathOperator{\minset}{min}
\def\fiireps{{\cal{R}}}

\newlength{\mlength} % Throwaway length.

% Type of convergence. We want all arrows to have the same length, hence the
% boxes.
\newlength{\convarrowwidth}
\settowidth{\convarrowwidth}{\scriptsize p.w.} % Put in the longest superscript
\def\converges{\xrightarrow{  \mathmakebox[\convarrowwidth]{}  }}
\def\convp{\xrightarrow{  \mathmakebox[\convarrowwidth]{p}  }}
\def\convd{\xrightarrow{  \mathmakebox[\convarrowwidth]{d}  }}
\def\convm^#1{\xrightarrow{  \mathmakebox[\convarrowwidth]{L^{#1}}  }}
\def\convpw{\xrightarrow{  \mathmakebox[\convarrowwidth]{p.w.}  }}

\def\pmf{{pmf}\xspace} % Abbrev. for prob. mass function
\def\cdf{{cdf}\xspace} % Abbrev. for cumulative distribution function

\usepackage{stmaryrd}
\def\Iver#1{ \llbracket #1 \rrbracket }


% Common width measures
\newcommand{\widthm}[1]{ \mathbf{#1} } % Width measure style
\DeclareMathOperator{\tw}{ \widthm{tw} }
\DeclareMathOperator{\pw}{ \widthm{pw} }
\DeclareMathOperator{\td}{ \widthm{td} }
\DeclareMathOperator{\cw}{ \widthm{cw} }
\DeclareMathOperator{\rw}{ \widthm{rw} }
\DeclareMathOperator{\wm}{ \widthm{wm} } % Generic width measure
\DeclareMathOperator{\width}{ \widthm{width} } % Generic width function for decompositions

% Protrusions
\def\YYYY{{Y_0 \uplus Y_1 \uplus \cdots \uplus Y_\ell}} % I don't want to type this anymore
\WithSuffix\def\YYYY'{{Y'_0 \uplus Y'_1 \uplus \cdots \uplus Y'_{\ell'}}} 
\def\protrusion#1{protrusion$^{#1}$}


% Basic graph things
\def\indeg{d^{-}}
\def\outdeg{d^{-}}
\def\mindeg{\delta}
\def\minindeg{\delta^-}
\def\avgdeg{\overbar d}
\def\avgindeg{\overbar d^{\,-}}
\def\avgoutdeg{\overbar d^+}
\def\maxdeg{\Delta}
\def\maxindeg{\Delta^{\!-}}

% Graph parameters & modulators
\def\twmod{\tw^\Delta} 
\def\tdmod{\td^\Delta}
\newcommand{\ds}{\mathop{\mathbf{ds}}}

\def\fii{finite integer index\xspace} 

% Words and abbreviations I have yet to decide how to
% typeset them
\def\FII{FII\xspace}
\def\FI{FI\xspace}
\def\YES{YES\xspace} % As in YES-instance
\def\NO{NO\xspace} % As in NO-instance

\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\yay}{\ding{51}}%
\newcommand{\yaay}{\kern4pt \ding{51} \kern-8pt \ding{51}}%
\newcommand{\nay}{\color{black!33}\ding{55}}%

\newcommand{\nab}{\mathop{\triangledown}}
\newcommand{\topnab}{\mathop{\widetilde \triangledown}}
\newcommand{\dist}{\ensuremath{\text{dist}}}

\newcommand{\numcliques}{\ensuremath{\mathop{\#\omega}}}
\newcommand{\randgr}[2]{\ensuremath{\mathcal{G}_{#1}(#2)}}
\newcommand{\prob}[1]{\ensuremath{\mathbf{Pr}\left [ #1 \right ]}}


\def\any{\mathord{\color{black!33}\bullet}}%
\def\anyrel{\mathbin{\color{black!33}\blacklozenge}}%
\def\anyleq{\mathbin{\color{black!33}\blacktriangleleft}}%
\def\anygeq{\mathbin{\color{black!33}\blacktriangleright}}%
\def\notanyleq{\mathbin{\not \color{black!33}\blacktriangleleft}}%


% Tree/Graph functions & operators
\def\comps{\operatorname{K}} % Conn. comps of a graph
\def\root{\operatorname{root}} % Root of a tree
\def\rpath{\operatorname{rpath}} % Path from node to root in tree
\def\leaves{\operatorname{leaves}} % Leaves of a tree
\def\inner{\operatorname{inner}} % Inner nodes of a tree
\def\depth{\operatorname{depth}}
\def\height{\operatorname{height}}
\def\anc{\operatorname{anc}}
\def\desc{\operatorname{desc}}
\def\clos{\operatorname{clos}} % Closure of a rooted tree
\def\lca{\operatorname{lca}}
\def\lcaclos{\clos^{\lca}}

\def\diam{\mathop{diam}} % Graph diameter
\def\radius{\mathop{rad}} % Graph radius

% Functions
\def\domain{\operatorname{dom}}
\def\image{\operatorname{img}}
\def\conv{ \mathbin{ \ast } } % Convolution
\def\compose{ \mathbin{ \circ } } % Composition

% Floor and ceiling brackets
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

% Arg min, arg max
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% Define theorems etc.
\theoremstyle{plain}
\newtheorem{lemma}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\newtheorem{proposition}{Proposition}
\newtheorem*{claim}{Claim}

\newtheoremstyle{case}
  {\topsep}   % ABOVESPACE
  {\topsep}   % BELOWSPACE
  {}  % BODYFONT
  {\parindent}       % INDENT (empty value is the same as 0pt)
  {\bfseries} % HEADFONT
  {\normalfont.}         % HEADPUNCT
  {5pt plus 1pt minus 1pt} % HEADSPACE
  {#1 #2: {\normalfont #3}}          % CUSTOM-HEAD-SPEC

\theoremstyle{case}
\newtheorem{case}{Case}
\newtheorem{subcase}{Case}
\numberwithin{subcase}{case}
\makeatletter%Make sure case-counter is reset in every environment
\@addtoreset{case}{lemma}
\@addtoreset{case}{theorem}
\@addtoreset{case}{corollary}
\@addtoreset{case}{claim}
\makeatother

\theoremstyle{definition}
\newtheorem{redrule}{Reduction Rule}
\newtheorem{definition}{Definition}

% Abbreviations, typographically correct
\newcommand*{\WLOG}{w.l.o.g\xperiod}
       % \wlog is defined in verbatim.sty for some reason.
\newcommand*{\WWLOG}{W.l.o.g\xperiod}
\renewcommand*\etal{\xperiodafter{\emph{et~al}}}
\newcommand*{\wrt}{w.r.t.\xperiod}
\newcommand{\ditto}{\textbf{-- \raisebox{-3pt}{''} --}}%

% Rules
\newcommand*\varrule[1][0.4pt]{\leavevmode\leaders\hrule height#1\hfill\kern0pt}

% notes, todo, remarks
\newcommand\Color[2]{\textcolor{#1}{#2}}
\newcommand{\nb}[1]{\marginpar{\scriptsize #1}}

% Tyopgraphic tweaks
\renewcommand{\labelitemi}{\parbox[c]{.4em}{\small\textbullet}}

\setlist[1]{labelindent=\parindent,leftmargin=*} 
\setlist{itemsep=0pt}
\setitemize[1]{label={\small\textbullet}}

% Centering without extra whitespace
\newenvironment{tightcenter}
 {\parskip=0pt\par\nopagebreak\centering}
 {\par\noindent\ignorespacesafterend}

% Problem environment
\usepackage{ctable}
\newlength{\RoundedBoxWidth}
\newsavebox{\GrayRoundedBox}
\newenvironment{GrayBox}[1]%
   {\setlength{\RoundedBoxWidth}{\textwidth-4.5ex}
    \def\boxheading{#1}
    \begin{lrbox}{\GrayRoundedBox}
       \begin{minipage}{\RoundedBoxWidth}%
   }{%
       \end{minipage}
    \end{lrbox}%
    \begin{tightcenter}%
    \begin{tikzpicture}%
       \node(Text)[draw=black!20,fill=white,rounded corners,%
             inner sep=2ex,text width=\RoundedBoxWidth]%
             {\usebox{\GrayRoundedBox}};
        \coordinate(x) at (current bounding box.north west);
        \node [draw=white,rectangle,inner sep=3pt,anchor=north west,fill=white] 
        at ($(x)+(6pt,.75em)$) {\boxheading};
    \end{tikzpicture}
    \end{tightcenter}\vspace{0pt}%
    \ignorespacesafterend
}    

\newenvironment{problem}[2][]{\noindent\ignorespaces%
                                \FrameSep=6pt%
                                \parindent=0pt%
                \vspace*{-.5em}
                \ifthenelse{\isempty{#1}}{%
                  \begin{GrayBox}{\textsc{#2}}%                
                }{%
                  \begin{GrayBox}{\textsc{#2} parameterized by~{#1}}%  
                }
                \index[prob]{#2|textbf}%
                \newcommand\Prob{Problem:}%
                \newcommand\Input{Input:}%                        
                \begin{tabular*}{\textwidth}{@{\hspace{.1em}} >{\itshape} p{1.6cm} p{0.8\textwidth} @{}}%        
            }{
                \end{tabular*}%
                \end{GrayBox}%
                \vspace*{-.5em}
                \ignorespacesafterend
            }                 

% Draft & Old environment
\renewenvironmentx{leftbar}[2][1=0.5pt, 2=5pt]{% 
  \def\FrameCommand{\vrule width #1 \hspace{#2}}\MakeFramed {\advance\hsize-\width \FrameRestore}}%
{\endMakeFramed}
\newenvironment{draft}[1]{%
                \color{gray}%
                \begin{leftbar}%                
                \begin{center}\emph{Draft:} {#1}\end{center}
            }{
                \end{leftbar}%
             }

\newenvironment{old}{
  \color{gray}%
  \begin{leftbar}%  
}{
  \end{leftbar}%
}


% Sweepline
\def\sweepline{  \begin{center}{\color{black!50}\rule{5cm}{.5pt}}\end{center} }

\newcommand*\circled[4]{\tikz[baseline=(char.base)]{
             \node[circle,fill=#3,draw=#4,draw,inner sep=1pt,minimum size=1.2em] (char) {\color{#2} #1};}}

% Tikz hacks
% \def\showbounds{% Shows bounding box of tikz picture.
%     {\draw[color=red] (current bounding box.north west) -- (current bounding box.north east);
%     \draw[color=red] (current bounding box.north east) -- (current bounding box.south east);
%     \draw[color=red] (current bounding box.south east) -- (current bounding box.south west);
%     \draw[color=red] (current bounding box.south west) -- (current bounding box.north west);}
% }

% computes width and height of tikzpicture
% \makeatletter
% \newcommand{\pgfsize}[2]{ % #1 = width, #2 = height
%  \pgfextractx{\@tempdima}{\pgfpointdiff{\pgfpointanchor{current bounding box}{south west}}
%  {\pgfpointanchor{current bounding box}{north east}}}
%  \global#1=\@tempdima
%  \pgfextracty{\@tempdima}{\pgfpointdiff{\pgfpointanchor{current bounding box}{south west}}
%  {\pgfpointanchor{current bounding box}{north east}}}
%  \global#2=\@tempdima
% }
% \makeatother

% Simulated float
\newlength{\wleft}  \newlength{\wright}
\newcommand{\minifloat}[3]{ % #1 = ratio left/right, #2 = left content, #3 = right content
  \th{\wleft}{#1\linewidth}
  \setlength{\wright}{\linewidth}
  \addtolength{\wright}{-\wleft}
  \noindent\begin{minipage}{\wleft}%
    #2
  \end{minipage}%
  \begin{minipage}{\wright}%
    #3
  \end{minipage}
}

% The following is a suggestion from 
% http://mintaka.sdsu.edu/GF/bibliog/latex/floats.html
%   General parameters, for ALL pages:
\renewcommand{\topfraction}{0.9}  % max fraction of floats at top
\renewcommand{\bottomfraction}{0.8} % max fraction of floats at bottom
%   Parameters for TEXT pages (not float pages):
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}     % 2 may work better
\setcounter{dbltopnumber}{2}    % for 2-column pages
\renewcommand{\dbltopfraction}{0.9} % fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}  % allow minimal text w. figs
%   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.7}  % require fuller float pages
% N.B.: floatpagefraction MUST be less than topfraction !!
\renewcommand{\dblfloatpagefraction}{0.7} % require fuller float pages


% Helpers
\newenvironment{todolist}{ 
      \todo{Finish list.}
      \def\urgent{\item[\circled{!}{White}{Red}{Red}]}
      \def\maybe{\item[\circled{?}{White}{RoyalBlue}{RoyalBlue}]}
      \def\task{\item[\circled{$\star$}{White}{RoyalBlue}{RoyalBlue}]}
      \color{RoyalBlue}\small
      \begin{compactitem}[$\ast$]
    }{
      \end{compactitem}
    }

\def\todocite{{\color{Red}[Citation needed!]}\todo{}}
\def\todoprove{\color{Red}\todo{Proof unfinished.}}
\def\todoimprove{\color{Blue}\todo{Check whether okay (notation, style \etc).}}
\def\todofluff{\centerline{\color{Magenta} (You need to write some fluff here.)}\todo{Fluff.}}

% Fix references in description environment:
% a \label will now be referenced by the description title
% instead of an internal number.
% \makeatletter
% \let\orgdescriptionlabel\descriptionlabel
% \def\@savelabel{}
% \renewcommand*{\descriptionlabel}[1]{%
%   \let\orglabel\label
%   \let\label\@gobble
%   \phantomsection
%   \def\@savelabel{#1}
%   \edef\@currentlabel{{\def\hfil{}#1}}% Dirty trick because this adds a \hfil at the end
%   \edef\@currentlabelname{#1}%
%   \let\label\orglabel
%   \orgdescriptionlabel{#1}%
% }
% \makeatother
\makeatletter
\def\namedlabel#1#2{\begingroup
   \def\@currentlabel{#1}%
   \label{#2}\endgroup
}
\makeatother

% Hyphenation
\usepackage{hyphenat}
\hyphenation{tree-depth tree-width path-width analy-sis white-space pro-gramm-ing}

% Hard-to-type names
\def\Nesetril{Ne\v{s}et\v{r}il\xspace}
\def\Zdenek{Zden\v{e}k\xspace}
\def\Dvorak{Dvo\v{r}\'{a}k\xspace}
\def\Kral{Kr\'{a}l\xspace}
\def\Erdos{Erd\H{o}s\xspace}
\def\Renyi{R\'{e}nyi\xspace}
\def\Barabasi{Barab\'{a}si\xspace}
\def\Bollobas{Bollob\'{a}s\xspace}
\def\Szemeredi{Szemer\'{e}di\xspace}

% Special environemnt to typeset the no-FII tables
\usepackage{environ}% 
\NewEnviron{nofiitable}{\noindent\ignorespaces%
  \newcommand{\result}[2]{%
    \cline{1-3} \cline{5-7}%
    \multicolumn{3}{r}{##1} && \multicolumn{3}{r}{##2}%
  }
  \[\arraycolsep=1.4pt\def\arraystretch{1.3}%
  \begin{array}{rcr p{1cm} rcr}
    \BODY
  \end{array}
  \]
}

% New columntypes for tables
% Define this last since the last def messed up the syntax highlighting ><
\newcolumntype{m}{>{$}l<{$}}
\newcolumntype{M}{>{$\displaystyle}l<{$}} 

%%% Local Variables: 
%%% TeX-command-default: "Make"
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

